Generalized Presentation Attack Detection: a face anti-spoofing evaluation proposal

Over the past few years, Presentation Attack Detection (PAD) has become a fundamental part of facial recognition systems. Although much effort has been devoted to anti-spoofing research, generalization in real scenarios remains a challenge. In this paper we present a new open-source evaluation framework to study the generalization capacity of face PAD methods, coined here as face-GPAD. This framework facilitates the creation of new protocols focused on the generalization problem establishing fair procedures of evaluation and comparison between PAD solutions. We also introduce a large aggregated and categorized dataset to address the problem of incompatibility between publicly available datasets. Finally, we propose a benchmark adding two novel evaluation protocols: one for measuring the effect introduced by the variations in face resolution, and the second for evaluating the influence of adversarial operating conditions.

==> one_pai.tex <==
% This table is not used in the paper. Neverthless, the results of this experiments are mentioned.

\begin{table*}[]
\begin{tabular}{c|c|c|}
\cline{2-3}
\multicolumn{1}{l|}{}                                & Protocol       & HTER (\%) \\ \hline
\multicolumn{1}{|c|}{\multirow{3}{*}{Quality-Based}} & One-PAI-Print  & 14.53     \\ \cline{2-3} 
\multicolumn{1}{|c|}{}                               & One-PAI-Replay & 10.22     \\ \cline{2-3} 
\multicolumn{1}{|c|}{}                               & One-PAI-Mask   & 10.08     \\ \hline
\multicolumn{1}{|c|}{\multirow{3}{*}{Color-Based}}   & One-PAI-Print  & 4.41      \\ \cline{2-3} 
\multicolumn{1}{|c|}{}                               & One-PAI-Replay & 3.92      \\ \cline{2-3} 
\multicolumn{1}{|c|}{}                               & One-PAI-Mask   & 2.90      \\ \hline
\end{tabular}
\end{table*}

==> protocols_categories.tex <==
\begin{table}[htbp]
\tiny
\centering
\begin{tabular}{ccc|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\cline{4-24}
                                                                                                           &                                                                            &                                                 & \multicolumn{21}{c|}{Categorization}                                                                                                                                                                                                                                                                                                                                                                                                                                                                     \\ \hline
\multicolumn{1}{|c|}{\multirow{3}{*}{Proposed Protocols}}                                                  & \multicolumn{1}{c|}{\multirow{3}{*}{Subsets}}                              & \multirow{3}{*}{Samples}                        & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Common \\ Face Resolution\end{tabular}} & \multicolumn{9}{c|}{\begin{tabular}[c]{@{}c@{}}Common \\ PAI\end{tabular}}           & \multicolumn{6}{c|}{\begin{tabular}[c]{@{}c@{}}Common \\ Capture Devices\end{tabular}}                                                                                                     & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Common\\ Lightning\end{tabular}}                                             \\ \cline{4-24} 
\multicolumn{1}{|c|}{}                                                                                     & \multicolumn{1}{c|}{}                                                      &                                                 & \multirow{2}{*}{sf}         & \multirow{2}{*}{mf}         & \multirow{2}{*}{bf}        & \multicolumn{3}{c|}{print} & \multicolumn{3}{c|}{replay} & \multicolumn{3}{c|}{mask} & \multicolumn{2}{c|}{webcam} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}mobile\\ tablet\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}digital\\ camera\end{tabular}} & \multirow{2}{*}{controlled} & \multirow{2}{*}{adverse} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}no\\ info\end{tabular}} \\ \cline{7-21}
\multicolumn{1}{|c|}{}                                                                                     & \multicolumn{1}{c|}{}                                                      &                                                 &                             &                             &                            & l       & m       & h      & l        & m       & h      & l       & m      & h      & l            & h            & l                                     & h                                    & l                                      & h                                    &                             &                          &                                                                    \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Cross Face Resolution\\ (1)\end{tabular}}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Train \\  Dev\end{tabular}} & \begin{tabular}[c]{@{}c@{}}NN\\ NN\end{tabular} & X                           & X                           &                            & X       & X       & X      & X        & X       & X      & X       & X      & X      & X            & X            & X                                     & X                                    & X                                      & X                                    & X                           & X                        & X                                                                  \\ \cline{2-24} 
\multicolumn{1}{|c|}{}                                                                                     & \multicolumn{1}{c|}{Test}                                                  & NN                                              &                             &                             & X                          & X       & X       & X      & X        & X       & X      & X       & X      & X      & X            & X            & X                                     & X                                    & X                                      & X                                    & X                           & X                        & X                                                                  \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Cross Face Resolution\\ (2)\end{tabular}}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Train\\ Dev\end{tabular}}   & \begin{tabular}[c]{@{}c@{}}NN\\ NN\end{tabular} &                             &                             & X                          & X       & X       & X      & X        & X       & X      & X       & X      & X      & X            & X            & X                                     & X                                    & X                                      & X                                    & X                           & X                        & X                                                                  \\ \cline{2-24} 
\multicolumn{1}{|c|}{}                                                                                     & \multicolumn{1}{c|}{Test}                                                  & NN                                              & X                           & X                           &                            & X       & X       & X      & X        & X       & X      & X       & X      & X      & X            & X            & X                                     & X                                    & X                                      & X                                    & X                           & X                        & X                                                                  \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Adverse Condition\\ (1)\end{tabular}}}     & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Train\\ Dev\end{tabular}}   & \begin{tabular}[c]{@{}c@{}}NN\\ NN\end{tabular} &                             &                             & X                          &         &         & X      &          &         & X      &         &        & X      &              & X            &                                       & X                                    &                                        & X                                    & X                           &                          &                                                                    \\ \cline{2-24} 
\multicolumn{1}{|c|}{}                                                                                     & \multicolumn{1}{c|}{Test}                                                  & NN                                              & X                           & X                           &                            & X       & X       &        & X        & X       &        & X       & X      &        & X            &              & X                                     &                                      & X                                      &                                      &                             & X                        &                                                                    \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Adverse Condition\\ (2)\end{tabular}}}     & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Train\\ Dev\end{tabular}}   & \begin{tabular}[c]{@{}c@{}}NN\\ NN\end{tabular} & X                           & X                           &                            & X       & X       &        & X        & X       &        & X       & X      &        & X            &              & X                                     &                                      & X                                      &                                      &                             & X                        &                                                                    \\ \cline{2-24} 
\multicolumn{1}{|c|}{}                                                                                     & \multicolumn{1}{c|}{Test}                                                  & NN                                              &                             &                             & X                          &         &         & X      &          &         & X      &         &        & X      &              & X            &                                       & X                                    &                                        & X                                    & X                           &                          &                                                                    \\ \hline
\end{tabular}
\end{table}
